Massively Parallel Algorithms for Approximate Shortest Paths

We present fast algorithms for approximate shortest paths in the massively parallel computation (MPC) model. We provide randomized algorithms that take $poly(\log{\log{n}})$ rounds in the near-linear memory MPC model. Our results are for unweighted undirected graphs with $n$ vertices and $m$ edges. Our first contribution is a $(1+\epsilon)$-approximation algorithm for Single-Source Shortest Paths (SSSP) that takes $poly(\log{\log{n}})$ rounds in the near-linear MPC model, where the memory per machine is $\tilde{O}(n)$ and the total memory is $\tilde{O}(mn^{\rho})$, where $\rho$ is a small constant. Our second contribution is a distance oracle that allows to approximate the distance between any pair of vertices. The distance oracle is constructed in $poly(\log{\log{n}})$ rounds and allows to query a $(1+\epsilon)(2k-1)$-approximate distance between any pair of vertices $u$ and $v$ in $O(1)$ additional rounds. The algorithm is for the near-linear memory MPC model with total memory of size $\tilde{O}((m+n^{1+\rho})n^{1/k})$, where $\rho$ is a small constant. While our algorithms are for the near-linear MPC model, in fact they only use one machine with $\tilde{O}(n)$ memory, where the rest of machines can have sublinear memory of size $O(n^{\gamma})$ for a small constant $\gamma < 1$. All previous algorithms for approximate shortest paths in the near-linear MPC model either required $\Omega(\log{n})$ rounds or had an $\Omega(\log{n})$ approximation. Our approach is based on fast construction of near-additive emulators, limited-scale hopsets and limited-scale distance sketches that are tailored for the MPC model. While our end-results are for the near-linear MPC model, many of the tools we construct such as hopsets and emulators are constructed in the more restricted sublinear MPC model.

==> comments.tex <==
fixed:

Page 1:
        - "that receives a lot of attention" -> "which has received a lot of attention" - fixed (2 places)
Page 2:
        - When comparing to previous work, I would suggest mentioning that much of this work holds even for weighted graphs.  So while it is true that all previous algorithms for SSSP required either log rounds or log approximation even in the unweighted setting, this feels somewhat unfair, since at least some of this previous work actually handles the more general weighted setting with the same bounds.

updated: "All these algorithms work in the more restricted sublinear MPC model, *and work in weighted graphs*"

In particular, our algorithm is exponentially faster compared to previous algorithms for $(1+\epsilon)$-approximate SSSP \cite{li2020faster, andoni2020parallel} *that worked also for weighted graphs*.

multiplicative *weighted* $\Omega(\log{n})$-spanner

allow to query approximate distances in $O(1)$ rounds *in weighted graphs*

our algorithm gives a better $O(1)$-approximation. *We remark that the previous works also handle weighted graphs*.

Page 3:
        - When defining a hopset, you define it just as a set of edges and talk about distance in G'.  This only makes sense if the lengths of the hopset edges are either explicitly defined (which you don't do) or implicitly defined as the shortest path between the endpoints.  So I think you need to mention that hopset edges come with lengths (either implicit or explicit).

updated: A hopset is a set of *weighted* edges

Page 6:
        - You define \rho to be a constant in [1/log log n, 1/2].  It seems odd to call \rho a constant but then allow it to be a function of n (e.g., 1/log log log n). 

I think it's ok to keep it like this

Page 8:
        - There are some typos and undefined notation at the beginning of Section 3. I don't think that \ell has been defined. and the first place that you say \frac12 \alpha \epsilon \ell, I think you mean \frac12 \alpha(1/\epsilon)^{\ell}.
        - "in sequel" -- I'm not sure what you mean by this.  "in the following section"?


updated: we assume access to a $(1+\epsilon_H, \beta)$-hopset $H$ for distances up to %$\frac{1}{2}\alpha\epsilon \ell$ 
 *$\frac{1}{2}\alpha\eps{\ell}$* in the graph $G$ *for a suitable parameter $\ell$*

for a suitable parameter $\ell$ that will be specified *in the following section.*

Page 9:
        - The second paragraph of Section 3.1 is quite confusing.  It talk about the memory necessary per phase, but nothing like that seems to appear in Algorithm 1.  I think you are actually talking about phases of a *different* algorithm (Algorithm 2), but that algorithm has not been introduced yet.
        - The definition of B(n) involves a parameter \beta.  Is this the same as \beta_H?

updated:

However, *during our algorithm we will work in phases where* the execution of each phase $i$ requires using $\tilde{O}(deg_i)$ memory per edge in $E\cup H$. 

changed beta_H to beta in this section (appeared a few times)

Page 17:
        - In Lemma 3.10, has i_0 been defined?  It's clear from context what it is, but I don't remember it being defined earlier.

updated (it was defined much earlier):
In the following two lemmas, we provide an upper bound on the expected size of the set $A_i$ for all $i\in [0,\ell]$. *Recall that for every $i\in [0,i_0 =\izo]$, we set $deg_i = \degi$, and for every $i\in [i_0+1,\ell]$ we set $deg_i = n^\rho$.*



==> emulators.tex <==

In this section, we show how the general framework from Section \ref{sec general} can be used for the construction of near-additive emulators. 
We are given an unweighted, undirected graph $G=(V,E)$  on $n$ vertices, parameters $\epsilon <1/10$, $\rho \in[ 1/{\log {\log n}}, 1/2]$ and $\kappa \geq 1/\rho$. In addition, we are given a $(1+\epsilon_H,\beta_H)$-hopset $H$ for distances up to $\eps{\emuell}$ in the graph $G$. 
We set $\alpha = 1$. This input is provided to the algorithm described in Section \ref{sec general}. Denote by $EM$ the output of the algorithm. 

Corollary \ref{coro Q} provides a straightforward upper bound on both the size of the output $EM$ as well as the round complexity of the algorithm. It is left to show that the set $EM$ is indeed a near-additive emulator. By Corollary \ref{coro Q},  for $\ell = \emuell$, we have for every pair of vertices $u,v\in V$  with $d_G(u,v)\leq \eps{\ell}$ 
    
    \begin{equation}\label{eq emu st}
    \begin{array}{lclclclclc}
        d_G(u,v)&\leq& d_{EM}(u,v) 
        %&\leq&d^{(6(\frac{1}{\epsilon}+3)^{\ell})}_{EM} (u,v)\\&& 
        &\leq& (1+\epsilon_H +28\epsilon \ell ) d_G(u,v) +28\cdot \eps{\ell-1}  .
    \end{array}
    \end{equation}

This relation may seem unsatisfactory at first, as it does not explicitly provide an upper bound on the stretch for distant pairs of vertices. However, in the following lemma, we show that eq. \ref{eq emu st} is enough to show that the set $Q$ provides $(1+\epsilon_{EM},\beta_{EM})$-approximation for the distance of any pair of vertices $u,v\in V$.


\begin{lemma}
    \label{lemma st emu}
    For every pair of vertices $u,v\in V$, we have 
    \begin{equation*}
        \begin{array}{lclclclclclc}
             
        d_G(u,v)&\leq &  d_{EM}(u,v) &\leq& \left(1+\epsilon_H +28\epsilon (\ell+1)   \right) \cdot  {d_G(u,v)} +28 \eps{\ell-1} .
        \end{array}
    \end{equation*}
\end{lemma}
\begin{proof}
    Let $u,v \in V$, and let $\pi(u,v)$ be a shortest path between them in the graph $G$. Let $r = \left\lceil \frac{d_G(u,v)}{\eps{\ell}}\right\rceil $. We divide the path $\pi(u,v)$ into $r$ segments $S_1, S_2, \dots, S_{r}$, each of length exactly $\eps{\ell}$, except for the last segment which may be shorter. For every segment $S_i$, denote by $u_i$ its first vertex and $v_i$ its last vertex. Observe that for all $i\in [1,r-1]$ we have $v_i = u_{i+1}$. In addition, we also have $u= u_1$ and $v = v_{r}$.  See Figure \ref{fig emu} for an illustration. 

    \begin{figure}
        \centering
        \includegraphics[scale = 0.15]{Figures/uv_path_emu2.png}
        \caption{The $u-v$ path in $Q$. The solid straight line depicts the shortest path $\pi(u,v)$ in $G$. The dashed line depicts the division of $\pi(u,v)$ into segments. The dotted lines depict the path we have between the endpoints of each segment by  Corollary \ref{coro Q}.   }
        \label{fig emu}
    \end{figure}

    By Corollary \ref{coro Q}, we have that for every index $i\in [1,r]$, it holds that 
       \begin{equation*}
        \begin{array}{lclclclclclc}
             d_G(u_i,v_i)&\leq& d_{EM}(u_i,v_i) &\leq& (1+\epsilon_H +28\epsilon \ell ) d_G(u_i,v_i) +28\cdot \eps{\ell-1}  .
        
        \end{array}
    \end{equation*}
   In particular, we have $d_G(u_i,v_i)  \leq d_{EM} (u_i,v_i)$ for all $i\in [1,r]$, and thus 
    $d_G(u,v)\leq d_{EM}(u,v)$.

    Moreover, 
    \begin{equation*}
        \begin{array}{lclclclclclc}
             d_{EM}(u,v) &\leq & \sum_{i=1}^{r} d_{EM}(u_i,v_i) \\
             &\leq & \sum_{i=1}^{r} (1+\epsilon_H +28\epsilon \ell ) d_G(u_i,v_i) +28 \eps{\ell-1} \\


             &\leq &  (1+\epsilon_H +28\epsilon \ell ) d_G(u,v) + 
             \left\lceil \frac{d_G(u,v)}{\eps{\ell}} \right\rceil \cdot 28 \eps{\ell-1} \\
             
             &= &  (1+\epsilon_H +28\epsilon \ell ) d_G(u,v) + 
              28\epsilon \cdot d_G(u,v)+  28 \eps{\ell-1} \\

             
             & = &  (1+\epsilon_H +28\epsilon (\ell+1) ) d_G(u,v) +  28 \eps{\ell-1}. \\
                 
        \end{array}
    \end{equation*}
\end{proof}



\subsection{Rescaling} 
In this section we rescale $\epsilon$ to obtain a $(1+\epsilon_{EM},\beta_{EM})$-emulator. 

Let $\epsilon_{EM} =28\epsilon (\ell+1)$. The condition $\epsilon< 1/10$ is translated to 
${\epsilon_{EM}}/{28(\ell+1)}\leq 1/10$. We replace it with the stronger condition $\epsilon_{EM}<1/2$.  
The additive term $28 \eps{\ell-1}$ now translates to $28\left(\frac{28 (\ell+1)}{\epsilon_{EM}}\right)^{\ell-1}$.

Recall that $\ell = \emuell $ and  $\rho \geq 1/\kappa$. Then, $\ell \leq {\log (\kappa\rho)} + 1/\rho$. Denote 
\begin{equation*}
\begin{array}{lclcl}
    \beta_{EM} & = & \betaemu.
\end{array}
\end{equation*} 
For the hopset $H$, we need a hopset for distances up to 

\begin{equation*}
        \begin{array}{lclclclclc}
             
\eps{\emuell}& \leq & \left(\frac{1}{\epsilon}\right)^{{\log (\kappa\rho)}+1/\rho} &=&  \left(  \frac{28(\emuellb+1)}{\epsilon_{EM}}\right)^{\emuellb}  .

        \end{array}
    \end{equation*}
Thus, we use the hopset construction devised in Section \ref{sec hop}, and use it to build a hopset for distances up to $t = \newtval$.  Observe that 
\begin{equation*}
        \begin{array}{lclclclclc}
             
  \left(  \frac{28(\emuellb+1)}{\epsilon_{EM}}\right)^{\emuellb} &\leq & \newtval & = & t .

        \end{array}
    \end{equation*}
\todo{add here the size of $H$ and the hopbound}

By Corollary \ref{coro hop}, the hopset $H$ has hopbound 


%========
Let $G=(V,E)$ be an unweighted, undirected graph on $n$-vertices and let $\rho \in [2/{\log {\log n}},1],\epsilon_\mathcal{H}<1 $ and $t>1$ be input parameters.
    Our algorithm computes. w.h.p., a $(1+\epsilon_\mathcal{H},\beta_\mathcal{H})$-hopset for distances up to $t$ in the graph $G$, where 
    \begin{equation*}
        \begin{array}{lclclclclc}
               \beta_\mathcal{H} &=& O\left(\frac{{\log t}}{\epsilon_\mathcal{H}\rho}\right)^{\frac{2}{\rho} +1} . 
        \end{array}
    \end{equation*}
    The size of the hopset is  $\tilde{O}(n^{1+\rho/2})$, and the algorithm terminates within $O(\frac{\beta_\mathcal{H}{\log t}}{\rho\gamma})$ communication rounds when 
    using machines with $O(n^\gamma)$ memory, and $\tilde{O}(|E|\cdot n^{\rho})$ total memory.         
%=========


By Corollary \ref{coro Q} and Lemma \ref{lemma st emu}, we derive the following corollary.

\begin{corollary}
    \label{coro emu}
    Let $G=(V,E)$ be an unweighted, undirected graph on $n$ vertices, and let $\epsilon_{EM} <1/2$,  $\rho \leq 1/2$ and $\kappa \geq 1/\rho$ be parameters. Given a $(1+\epsilon_\mathcal{H},\beta_\mathcal{H})$-hopset for distances up to $ \left(  \frac{28(\emuellb+1)}{\epsilon_{EM}}\right)^{\emuellb}$ in the graph $G$, our algorithm constructs an emulator $EM$, such that w.h.p., for every pair of vertices $u,v\in V$   we have 
   \begin{equation*}
        \begin{array}{lclc}
            d_G(u,v) &\leq& d_{EM} (u,v) \leq (1+\epsilon_\mathcal{H} +\epsilon_{EM}) d_G(u,v) +\betaemu.
        \end{array}
    \end{equation*}
    The size of the emulator is, w.h.p., $\tilde{O}(\nfrac)$.
    
    
    The algorithm can be executed in $O(\beta/\gamma)$ 
    rounds of MPC using machines with $O(n^\gamma)$ memory and $\tilde{O}((|E|+|H|+|Q|)n^\rho)$ total memory
    
\end{corollary}





\todo{If we want to remove $t$ from these corollaries, we can say that the algorithm first builds the hopset and then if computes the emulator, which increases the running time (slightly) but it makes the statement clearer}

A special interest is in the case where $\kappa ={\log n}$ and $\rho \geq 1/{\log {\log n}}$. In this case, the emulator has near-linear size. The properties of the emulator under these conditions are summarized in the following theorem. 

\begin{theorem}
    \label{theo emulators}
    Let $G=(V,E)$ be an unweighted, undirected graph on $n$ vertices, and let $\epsilon_{EM} <1/2$,  $\rho \in[ 1/{\log {\log n}}, 1/2]$. Given a $(1+\epsilon_\mathcal{H},\beta_\mathcal{H})$-hopset for distances up to $ \left(  \frac{28(\emuellbk+1)}{\epsilon_{EM}}\right)^{\emuellbk}$ in the graph $G$, our algorithm constructs an emulator $EM$,    such that for every pair of vertices $u,v\in V$   we have 
    \begin{equation*}
        \begin{array}{lclc}
    d_G(u,v) &\leq& d_{EM} (u,v) \leq (1+\epsilon_\mathcal{H} +\epsilon_{EM}) d_G(u,v) +\betaemuk.
        \end{array}
    \end{equation*}
    %The expected size of the emulator is $\tilde{O}(n) $.
    %O( n \cdot {\log( \rho{\log n})})$. 
    %Moreover, 
    W.h.p., the size of the emulator is  $\tilde{O}(n) $, and  
    %$O(n\cdot {\log^2 n }\cdot {\log(\rho{\log n})})$.
    the algorithm can be executed in $\tilde{O}(\beta_\mch/\gamma) $ MPC rounds using $\tilde{O}(m\cdot n^\rho/\gamma)$ machines, each with $O(n^\gamma)$ memory. 
    %The expected number of rounds of the algorithm in $\mpcng$ is $\tilde{O}(\beta_\mch/\gamma) $ % $O(\beta_\mch \cdot {\log {\log n}}/\gamma)$ when using $O(|E|\cdot n^\rho)$ total memory. Also, if the algorithm uses $\tilde{O}(|E|\cdot n^\rho)$ memory, it requires $\tilde{O}(\beta_\mch/\gamma) $ % O(\beta_\mch\cdot {\log {\log n}}/\gamma)$ rounds of $\mpcng$, w.h.p. 
\end{theorem}
















\begin{comment}
Let $G=(V,E)$ be an unweighted, undirected graph on $n$-vertices and let $\epsilon <1/10$, $\kappa = 2,3,\dots$ and $ 1/\kappa <\rho < 1/2$ be input parameters. Intuitively, the parameter $\rho$ governs the memory usage of the algorithm, the parameter $\kappa$ governs the size of the emulator, and the parameter $\epsilon$ governs the multiplicative error of the emulator. 
Let $\epsilon_{EM} = O(\epsilon({\log (\kappa\rho)}+1/\rho))$, and let 
$\beta_{EM} = \betaemu$. \mtodoi{it's probably good to give the reader examples of parameter choices we will be interested in, I assume we are interested in the case that $\kappa$ is something like $\log{n}$ and $\rho$ is constant, and then we get something like $\beta_{EM}=O(\log{\log{n}}/\epsilon)^{O(\log{\log{n}})}$, and more importantly $\log{\beta_{EM}} = poly(\log{\log{n}})$}

Given a  $(1+\epsilon_\mathcal{H},\beta_\mathcal{H})$-hopset $\mathcal{H}$ for distances up to $\eps{\emuell}/2$ in the graph $G$, our algorithm computes a $(1+\epsilon_\mathcal{H} +\epsilon_{EM},\beta_{EM})$-emulator for the graph $G$. 

Essentially, our algorithm begins by sampling a hierarchy $A_0, A_1, \dots$ using the sampling procedure described in Section \ref{sec samp gen}. Then, it constructs a near-additive emulator using the procedure described in Section \ref{sec edge selec gen}. 


\paragraph{Sampling Hierarchy.}
%The algorithm begins by sampling a hierarchy $V= A_0 \supseteq A_1 \supset \dots $ using the sampling procedure described in Section \ref{sec samp gen}.

In order to use the sampling procedure, we fix the sampling probability sequence and set the parameter $\ell$. Define the degree sequence to be 
$deg_i = {\min\{\degi, n^{\rho} \ | \ i\geq 0\}}$.
Set $i_0 = \lfloor{\log{\kappa\rho}}\rfloor$. Observe that for all $i\in [0,i_0]$ we have $deg_i = \degi$, and for all $i \geq  i_0+1$ we have $deg_i = n^\rho$.
The parameter $\ell$ is set to be the minimal integer such that $n\cdot \Pi_{j=0}^{\ell-1} deg_j^{-1} \leq deg_\ell$. In the following lemma, we show that $\ell = \emuell$. 
\begin{lemma}
    \label{lemma emuell min}
    The minimal integer $\ell$ that satisfies $n\cdot \Pi_{j=0}^{\ell-1} deg_j^{-1} \leq deg_\ell$ is $\emuell$. 
\end{lemma}
\begin{proof}
     
    \begin{equation*}
        \begin{array}{lclclclclc}
             n\cdot \Pi_{j=0}^{\ell-1} deg_j^{-1} & = & n\cdot \left(\Pi_{j=0}^{i_0} n^{-\frac{2^i}{\kappa}} \right)  \cdot\left( \Pi_{j=i_0+1}^{\ell-1} n^{-\rho} \right) \\
             &= &  n\cdot \left( n^{-\sum_{j=0}^{i_0}\frac{2^i}{\kappa}} \right)  
             \cdot\left(  n^{-(\ell-i_0)\rho} \right) 
              \\
             &= &   n^{1-\frac{2^{i_0+1}-1}{\kappa} -(\ell-i_0)\rho}
             \\ 
             &\leq  &   n^{1-\frac{\kappa\rho-1}{\kappa} - (\ell-i_0)\rho}
             & = & n^{1+\frac{1}{\kappa} - (\ell-i_0+1)\rho}.   
        \end{array}
    \end{equation*}
    Thus, $\ell$ is the minimal integer such that $1+\frac{1}{\kappa} - (\ell-i_0+1)\rho \leq  \rho$. We have  
    
    \begin{equation*}
        \begin{array}{lclclclclc}
             1+\frac{1}{\kappa} - (\ell-i_0+1)\rho &\leq &  \rho &\iff\\

            i_0 + 1/\rho+\frac{1}{\kappa\rho}- 2&\leq & \ell  &\iff\\
             \izo +\frac{\kappa + 1}{\kappa\rho}- 2&\leq & \ell .
             
             
             
             \end{array}
    \end{equation*}


It follows that $\ell$ must be at least $\izo +\frac{\kappa + 1}{\kappa\rho}- 2$. Since $\ell$ must be an integer,  we have that $\ell = \emuell$.
    
\end{proof}

This completes the discussion on the sampling procedure. 
\paragraph{Constructing the Emulator.}

We now discuss how the edge selection procedure from Section \ref{sec general} is used to construct our emulator $B$. 
 
The input for Algorithm \ref{alg connect} is the graph $G$, the $(1+\epsilon_\mathcal{H},\beta_\mathcal{H})$-hopset $ \mathcal{H}$ for distances up to $\eps{\ell}/2$, as well as the parameters $\epsilon_\mathcal{H},\beta_\mathcal{H}$, the parameter $\ell = \emuell$, the degree sequence 
$deg_i = {\min\{\degi, n^{\rho} \ | \ i\in [0,\ell]\}}$, the parameter $\alpha =1$ and the sampled hierarchy $A_0,\dots,A_{\ell+1}$. Let $EM$ be the output of the algorithm. This completes the description of the construction of our emulator $EM$.

\subsection{Size} 
In this section, we provide an upper bound on the size of $EM$. 

\begin{lemma}\label{lemma size emu}
    The size of the set $EM$ is $  O({\ln n}{\log (\kappa\rho)}\nfrac) $, w.h.p. 
\end{lemma}
\begin{proof}

Corollary \ref{coro Q}  implies that given the parameter $\ell = \emuell$ and  the sampling probability sequence $deg_i = {\min\{\degi, n^{\rho} \ | \ i\in [0,\ell]\}}$, the  size of the set $S$ of edges that may belong to the output of Algorithm \ref{alg connect} is, w.h.p., at most 
\begin{equation}
    \label{eq exp size Q emu}
        \begin{array}{lclclclclc}
        
        |S|  & =& O\left({\ln n}\cdot  n\sum_{i=0}^{\ell} deg_i\cdot \left(\Pi_{j=0}^{i-1} deg_j^{-1}\right)\right)  \\


        
        & = & O\left({\ln n}\left(
       n \sum_{i=0}^{i_0}\degi \cdot \left(\Pi_{j=0}^{i-1} n^{-\frac{2^j}{\kappa}} \right)          
        + n\sum_{i=i_0+1}^{\ell} n^\rho \cdot   \left(\Pi_{j=0}^{i_0} n^{-\frac{2^j}{\kappa}} \right)\cdot   \left(\Pi_{j=i_0+1}^{i-1} n^{-\rho}\right)\right)\right)
 \\



        & = & O\left({\ln n}\left(
       n \sum_{i=0}^{i_0}\degi \cdot  n^{-\frac{2^i-1}{\kappa}} 
        
        + n\sum_{i=i_0+1}^{\ell} n^\rho \cdot   n^{-\frac{2^{i_0+1}-1}{\kappa}} \cdot    n^{-\rho(i-i_0-1)}\right)\right)\\

        & = & O\left({\ln n}\left(
       (i_0+1)\nfrac
        
        + n\sum_{i=i_0+1}^{\ell}    n^{-\frac{\kappa\rho-1}{\kappa}} \cdot    n^{-\rho(i-i_0-2)}\right)\right)\\

        & = & O\left({\ln n}\left(
       i_0\cdot \nfrac
        
        + \nfrac \sum_{i=i_0+1}^{\ell} (n^{\rho})^{-(i-i_0-1)}\right)\right)\\

        & = & O\left({\ln n}\cdot  i_0\cdot \nfrac\right),
        \end{array}
\end{equation}
where the last inequality holds because $n^\rho \geq 2$. 
Since $EM\subseteq S$, we also have that w.h.p. $|EM|= O({\ln n }\cdot {\log( \kappa\rho)}\cdot \nfrac)$.
\end{proof}







\end{comment}


